Hypergraph Partitioning With Embeddings

Problems in scientific computing, such as distributing large sparse matrix operations, have analogous formulations as hypergraph partitioning problems. A hypergraph is a generalization of a traditional graph wherein "hyperedges" may connect any number of nodes. As a result, hypergraph partitioning is an NP-Hard problem to both solve or approximate. State-of-the-art algorithms that solve this problem follow the multilevel paradigm, which begins by iteratively "coarsening" the input hypergraph to smaller problem instances that share key structural features. Once identifying an approximate problem that is small enough to be solved directly, that solution can be interpolated and refined to the original problem. While this strategy represents an excellent trade off between quality and running time, it is sensitive to coarsening strategy. In this work we propose using graph embeddings of the initial hypergraph in order to ensure that coarsened problem instances retrain key structural features. Our approach prioritizes coarsening within self-similar regions within the input graph, and leads to significantly improved solution quality across a range of considered hypergraphs. Reproducibility: All source code, plots and experimental data are available at https://sybrandt.com/2019/partition.

==> misc/bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/bios/justin}}]{Justin Sybrandt}
received his B.Sc. in Computer Science from Grove City College and will graduate May 2020 with a Ph.D. in Computer Science from Clemson University. His work is focused in latent representations of text and graphs, with an emphasis on understanding scientific literature. 
He has since begun work at Google Brain. Contact him at \href{mailto:jsybrandt@google.com}{jsybrandt@google.com}.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/bios/ruslan}}]{Ruslan Shaydulin}
received his B.Sc. in Applied Mathematics and Physics from Moscow Institute of Physics and Technology and is currently pursuing a Ph.D. in Computer Science at Clemson University. His work is focused on quantum and classical algorithms for combinatorial optimization and machine learning. Contact him at \href{mailto:rshaydu@clemson.edu}{rshaydu@clemson.edu}.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/bios/ilya}}]{Ilya Safro}
is an associate professor in the School of Computing and faculty scholar
in the School of Health Research, Clemson University. His research interests
include graph algorithms, machine learning, combinatorial scientific computing, and quantum-classical methods. Safro received a Ph.D. in applied mathematics and computer science from the Weizmann Institute of Science. Contact
him at \href{mailto:isafro@clemson.edu}{isafro@clemson.edu}.
\end{IEEEbiography}


==> sections/abridged_hypergraph_data.tex <==
\begin{table*}
  \begin{minipage}{0.5\textwidth}
    \centering
    \tiny
    \begin{tabular}{l*{6}{r}}
      \toprule
        $H$ & $|V|$ & $|E|$
        & \multicolumn{2}{c}{$V$ Deg.}
        & \multicolumn{2}{c}{$E$ Size}\\
        & &
        & Mean & Std.
        & Mean & Std. \\
      \midrule
as-caida&26475&16538&3.657&29.016&5.855&29.016 \\
baxter&30722&24255&3.528&5.359&4.469&5.359 \\
brainpc2&27606&27606&6.498&131.257&6.498&131.257 \\
c-39&9271&9271&14.757&41.233&14.757&41.233 \\
c-42&10471&10471&10.532&41.339&10.532&41.339 \\
c-43&11125&11125&11.117&72.602&11.117&72.602 \\
c-45&13206&13206&13.210&85.104&13.210&85.104 \\
c-46&14913&14913&8.744&42.022&8.744&42.022 \\
c-48&18354&18354&9.049&16.866&9.049&16.866 \\
c-49&21132&21132&7.431&14.452&7.431&14.452 \\
c-50&22401&22401&8.644&22.902&8.644&22.902 \\
c/lp Mixture W/ Noise&107776&69568&5.379&12.552&8.333&12.552 \\
c/lp Mixture&107776&69368&5.374&12.552&8.350&12.552 \\
ca-AstroPh&18479&17490&21.369&30.683&22.577&30.683 \\
ca-CondMat&22523&20760&8.194&10.671&8.890&10.671 \\
ca-HepPh&11670&10514&20.181&47.173&22.400&47.173 \\
cari&1200&400&127.333&178.662&382.000&178.662 \\
case9&14453&14453&10.238&105.257&10.238&105.257 \\
cit-HepPh&28093&29526&14.913&27.227&14.189&27.227 \\
cit-HepTh&22908&22610&15.294&43.314&15.496&43.314 \\
co9&22829&10694&4.799&5.264&10.245&5.264 \\
com-dblp-cmty&260998&13477&2.758&4.340&53.411&4.340 \\
coupled&11341&11317&8.685&30.083&8.704&30.083 \\
cq9&21503&9247&4.493&4.673&10.449&4.673 \\
cvxqp3&17500&17500&6.998&3.626&6.998&3.626 \\
deter0 Mixture&21872&7845&2.061&0.900&5.746&0.900 \\
e18&38601&24617&4.053&5.472&6.356&5.472 \\
email-Enron&35153&25481&10.140&33.809&13.989&33.809 \\
email-EuAll&60532&33292&3.765&24.650&6.846&24.650 \\
fome12&48920&24284&2.913&1.303&5.869&1.303 \\
hangGlider\_4&15561&15561&9.609&110.835&9.609&110.835 \\
hangGlider\_5&16011&16011&9.696&112.427&9.696&112.427 \\
hvdc1&24842&24842&6.440&2.936&6.440&2.936 \\
jnlbrng1&40000&40000&4.980&0.141&4.980&0.141 \\
lowThrust\_4&13562&13562&11.867&64.031&11.867&64.031 \\
lowThrust\_5&16262&16262&12.198&70.124&12.198&70.124 \\
lp\_ken Mixture&32418&19219&10.513&10.796&17.733&10.796 \\
lp\_ken\_13&42659&23393&2.157&0.542&3.933&0.542 \\
lp\_osa\_07&25067&1118&5.777&1.032&129.528&1.032 \\
lp\_pds\_10&49932&16239&2.149&0.424&6.607&0.424 \\
lpi\_bgindy Mixture&97920&30322&11.824&9.319&38.182&9.319 \\
lpi\_ceria3d Mixture&39600&35384&11.891&23.733&13.308&23.733 \\
lpi\_gosh&13356&3662&7.474&5.231&27.260&5.231 \\
lpi\_greenbea Mixture&50319&24711&12.288&9.328&25.023&9.328 \\
lpl3&33686&10655&2.979&0.184&9.418&0.184 \\
Many Graph Mixture W/ Noise&110703&55507&3.650&2.971&7.279&2.971 \\
Many Graph Mixture&110703&55307&3.645&2.970&7.296&2.970 \\
memplus&17758&17758&7.104&22.035&7.104&22.035 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \begin{minipage}{0.5\textwidth}
    \centering
    \tiny
    \begin{tabular}{l*{6}{r}}
      \toprule
        $H$ & $|V|$ & $|E|$
        & \multicolumn{2}{c}{$V$ Deg.}
        & \multicolumn{2}{c}{$E$ Size}\\
        & &
        & Mean & Std.
        & Mean & Std. \\
      \midrule
mod2&65990&34355&3.022&2.883&5.804&2.883 \\
model10&16819&4398&8.940&4.645&34.191&4.645 \\
mult\_dcop\_01&25019&24817&7.710&144.682&7.773&144.682 \\
mult\_dcop\_02&25019&24817&7.710&144.682&7.773&144.682 \\
mult\_dcop\_03&25019&24817&7.708&144.682&7.771&144.682 \\
nemsemm2&48857&6922&3.725&2.568&26.292&2.568 \\
nemswrld&28496&6512&6.743&5.108&29.507&5.108 \\
nsir&10055&4450&15.409&25.894&34.817&25.894 \\
nug08-3rd&29856&19728&4.971&3.505&7.523&3.505 \\
obstclae&39996&39996&4.941&0.418&4.941&0.418 \\
OPF\_3754&15435&15435&10.254&5.531&10.254&5.531 \\
p010&19081&10071&6.183&4.984&11.715&4.984 \\
p2p-Gnutella30&36345&9205&2.416&2.594&9.539&2.594 \\
p2p-Gnutella31&62023&15383&2.368&2.669&9.549&2.669 \\
pds10&16558&16558&9.038&7.258&9.038&7.258 \\
pltexpa&70364&26894&2.033&1.288&5.319&1.288 \\
psse0&11028&26694&9.286&6.075&3.836&6.075 \\
psse2&11028&28632&10.452&6.713&4.026&6.713 \\
rajat09&24482&24391&4.309&1.117&4.325&1.117 \\
rajat10&30202&30101&4.311&1.116&4.326&1.116 \\
rajat22&39801&38431&4.919&24.574&5.095&24.574 \\
rajat27&20540&19163&4.786&16.261&5.130&16.261 \\
release-flickr-links\_x0\_10&18612&18612&15.842&38.179&15.842&38.179 \\
release-youtube-links\_x0\_100&115782&115778&3.999&7.222&3.999&7.222 \\
release-youtube-links\_x0\_25&28945&28938&3.996&7.784&3.997&7.784 \\
release-youtube-links\_x0\_50&57891&57888&3.999&7.222&3.999&7.222 \\
sc205-2r&62422&35212&1.974&18.129&3.500&18.129 \\
scagr7-2r&46679&32846&2.574&35.334&3.658&35.334 \\
scfxm1-2b&33047&18266&3.337&6.509&6.038&6.509 \\
scsd8-2b&35910&5130&3.140&17.607&21.982&17.607 \\
scsd8-2c&35910&5130&3.140&17.607&21.982&17.607 \\
scsd8-2r&60550&8650&3.141&22.885&21.990&22.885 \\
sctap1-2b&33858&15390&2.937&17.447&6.462&17.447 \\
sctap1-2r&63426&28830&2.938&23.857&6.464&23.857 \\
soc-Epinions1&50328&31149&9.530&39.646&15.398&39.646 \\
soc-Slashdot0811&77355&70893&11.622&37.228&12.682&37.228 \\
soc-Slashdot0902&82159&71882&11.464&37.486&13.103&37.486 \\
soc-sign-Slashdot081106&64371&27753&7.783&32.163&18.051&32.163 \\
soc-sign-Slashdot090216&68836&30554&7.734&32.971&17.423&32.971 \\
soc-sign-Slashdot090221&69038&30670&7.761&33.115&17.471&33.115 \\
soc-sign-epinions&76359&42470&10.327&43.547&18.567&43.547 \\
south31&35885&17989&3.120&132.364&6.224&132.364 \\
stormg2-27&37485&14306&2.513&2.000&6.584&2.000 \\
torsion1&39996&39996&4.941&0.418&4.941&0.418 \\
ulevimin&46754&6394&3.515&2.714&25.703&2.714 \\
wiki-Vote&2355&3728&43.018&40.735&27.175&40.735 \\
world&66747&34106&2.974&2.751&5.820&2.751 \\
youtube&90581&18173&3.107&8.121&15.487&8.121 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \caption{
    Hypergraph Details.
    \label{tab:hypergraph_details}
  }
\end{table*}


==> sections/considered_impl.tex <==
\section{Experiments}

We implement our algorithm in both
KaHyPar~\cite{shhmss2016alenex}, the $n$-level partitioner, as well as
Zoltan~\cite{devine2006parallel}, the $\log n$-level partitioner. These two
partitioners are considered as other alternatives such as
PaToH~\cite{ccatalyurek2011patoh} and hMetis~\cite{karypis1998hmetis} do not
provide open source implementations. In each, embedding-based coarsening
consists of only a few hundred lines of code, demonstrating that both
partitioners are easily expandable for new coarsening algorithms. For ease of
development, we use singletons to manage the state of the embedding, and
overwrite functions related to scoring neighboring nodes during the coarsening
process. We additionally implement a partitioner independent prepossessing step
to convert a hypergraph into a star-expanded classical graph in order to apply
existing graph embedding techniques. The output of these graph embeddings is
supplied as an auxiliary input to the singleton embedding manager. Overall, this
separation of embedding and partitioning allows easy experimentation and
adaptation with respect to new and constantly changing embedding techniques.

An additional implementation note is necessary for managing embedding behavior
during the recursive bisection process of Zoltan, which identifies larger
numbers of partitions by iteratively solving the 2-partition problem on
iterative halves of the input hypergraph. Simply put, node indices during the
recursive bisection process are remapped to start at zero for each recursive
partitioning call, which requires the embedding singleton to access the logic of
this routine. KaHyPar, in contrast, solves the $k$-partitioning problem directly
at the point of initial solution, and does not perform recursive bisection, and
therefore does not require extra engineering. While important for any wishing to
implement embedding-based coarsening in the context of recursive bisection, this
technical detail does not modify the overall behavior of the proposed algorithm.

==> sections/hypergraph_data.tex <==
\begin{small}
\begin{longtable}{*{9}{l}}
\multirow{2}{*}{Hypergraph}
& \multirow{2}{*}{\# Node}
& \multirow{2}{*}{\# Edge}
& \multicolumn{3}{c}{Node Degree}
& \multicolumn{3}{c}{Edge Degree} \\
& &
& Med. & Mean & Std.
& Med. & Mean & Std. \\
\hline
\endhead
com-dblp-cmty&260998&13477&1&2.758&4.340&8&53.411&4.340 \\
release-youtube-links\_x0\_100&115782&115778&2&3.999&7.222&2&3.999&7.222 \\
Many Graph Mixture&110703&55307&4&3.645&2.970&4&7.296&2.970 \\
Many Graph Mixture W/ Noise&110703&55507&4&3.650&2.971&4&7.279&2.971 \\
c/lp Mixture&107776&69368&4&5.374&12.552&4&8.350&12.552 \\
c/lp Mixture W/ Noise&107776&69568&4&5.379&12.552&4&8.333&12.552 \\
lpi\_bgindy Mixture&97920&30322&8&11.824&9.319&6&38.182&9.319 \\
youtube&90581&18173&1&3.107&8.121&4&15.487&8.121 \\
soc-Slashdot0902&82159&71882&3&11.464&37.486&3&13.103&37.486 \\
soc-Slashdot0811&77355&70893&3&11.622&37.228&3&12.682&37.228 \\
soc-sign-epinions&76359&42470&2&10.327&43.547&4&18.567&43.547 \\
pltexpa&70364&26894&2&2.033&1.288&4&5.319&1.288 \\
soc-sign-Slashdot090221&69038&30670&2&7.761&33.115&5&17.471&33.115 \\
soc-sign-Slashdot090216&68836&30554&2&7.734&32.971&5&17.423&32.971 \\
world&66747&34106&1&2.974&2.751&3&5.820&2.751 \\
mod2&65990&34355&1&3.022&2.883&3&5.804&2.883 \\
soc-sign-Slashdot081106&64371&27753&2&7.783&32.163&5&18.051&32.163 \\
sctap1-2r&63426&28830&2&2.938&23.857&6&6.464&23.857 \\
sc205-2r&62422&35212&2&1.974&18.129&3&3.500&18.129 \\
p2p-Gnutella31&62023&15383&1&2.368&2.669&10&9.549&2.669 \\
scsd8-2r&60550&8650&2&3.141&22.885&20&21.990&22.885 \\
email-EuAll&60532&33292&1&3.765&24.650&2&6.846&24.650 \\
release-youtube-links\_x0\_50&57891&57888&3&3.999&7.222&3&3.999&7.222 \\
soc-Epinions1&50328&31149&2&9.530&39.646&4&15.398&39.646 \\
lpi\_greenbea Mixture&50319&24711&9&12.288&9.328&5&25.023&9.328 \\
lp\_pds\_10&49932&16239&2&2.149&0.424&5&6.607&0.424 \\
fome12&48920&24284&3&2.913&1.303&4&5.869&1.303 \\
nemsemm2&48857&6922&4&3.725&2.568&11&26.292&2.568 \\
ulevimin&46754&6394&3&3.515&2.714&14&25.703&2.714 \\
scagr7-2r&46679&32846&1&2.574&35.334&3&3.658&35.334 \\
lp\_ken\_13&42659&23393&2&2.157&0.542&3&3.933&0.542 \\
jnlbrng1&40000&40000&5&4.980&0.141&5&4.980&0.141 \\
obstclae&39996&39996&5&4.941&0.418&5&4.941&0.418 \\
torsion1&39996&39996&5&4.941&0.418&5&4.941&0.418 \\
rajat22&39801&38431&4&4.919&24.574&4&5.095&24.574 \\
lpi\_ceria3d Mixture&39600&35384&6&11.891&23.733&3&13.308&23.733 \\
e18&38601&24617&1&4.053&5.472&4&6.356&5.472 \\
stormg2-27&37485&14306&2&2.513&2.000&5&6.584&2.000 \\
p2p-Gnutella30&36345&9205&1&2.416&2.594&10&9.539&2.594 \\
scsd8-2b&35910&5130&2&3.140&17.607&20&21.982&17.607 \\
scsd8-2c&35910&5130&2&3.140&17.607&20&21.982&17.607 \\
south31&35885&17989&1&3.120&132.364&6&6.224&132.364 \\
email-Enron&35153&25481&3&10.140&33.809&5&13.989&33.809 \\
sctap1-2b&33858&15390&2&2.937&17.447&6&6.462&17.447 \\
lpl3&33686&10655&3&2.979&0.184&6&9.418&0.184 \\
scfxm1-2b&33047&18266&2&3.337&6.509&5&6.038&6.509 \\
lp\_ken Mixture&32418&19219&7&10.513&10.796&4&17.733&10.796 \\
baxter&30722&24255&1&3.528&5.359&3&4.469&5.359 \\
rajat10&30202&30101&5&4.311&1.116&5&4.326&1.116 \\
nug08-3rd&29856&19728&6&4.971&3.505&8&7.523&3.505 \\
release-youtube-links\_x0\_25&28945&28938&2&3.996&7.784&2&3.997&7.784 \\
nemswrld&28496&6512&6&6.743&5.108&8&29.507&5.108 \\
cit-HepPh&28093&29526&6&14.913&27.227&10&14.189&27.227 \\
brainpc2&27606&27606&4&6.498&131.257&4&6.498&131.257 \\
as-caida&26475&16538&2&3.657&29.016&2&5.855&29.016 \\
lp\_osa\_07&25067&1118&6&5.777&1.032&22&129.528&1.032 \\
mult\_dcop\_01&25019&24817&5&7.710&144.682&6&7.773&144.682 \\
mult\_dcop\_02&25019&24817&5&7.710&144.682&6&7.773&144.682 \\
mult\_dcop\_03&25019&24817&5&7.708&144.682&6&7.771&144.682 \\
hvdc1&24842&24842&6&6.440&2.936&6&6.440&2.936 \\
rajat09&24482&24391&5&4.309&1.117&5&4.325&1.117 \\
cit-HepTh&22908&22610&6&15.294&43.314&11&15.496&43.314 \\
co9&22829&10694&2&4.799&5.264&4&10.245&5.264 \\
ca-CondMat&22523&20760&5&8.194&10.671&6&8.890&10.671 \\
c-50&22401&22401&4&8.644&22.902&4&8.644&22.902 \\
deter0 Mixture&21872&7845&2&2.061&0.900&4&5.746&0.900 \\
cq9&21503&9247&2&4.493&4.673&4&10.449&4.673 \\
c-49&21132&21132&4&7.431&14.452&4&7.431&14.452 \\
rajat27&20540&19163&3&4.786&16.261&4&5.130&16.261 \\
p010&19081&10071&2&6.183&4.984&4&11.715&4.984 \\
release-flickr-links\_x0\_10&18612&18612&11&15.842&38.179&11&15.842&38.179 \\
ca-AstroPh&18479&17490&10&21.369&30.683&11&22.577&30.683 \\
c-48&18354&18354&4&9.049&16.866&4&9.049&16.866 \\
memplus&17758&17758&4&7.104&22.035&4&7.104&22.035 \\
cvxqp3&17500&17500&6&6.998&3.626&6&6.998&3.626 \\
model10&16819&4398&11&8.940&4.645&11&34.191&4.645 \\
pds10&16558&16558&7&9.038&7.258&7&9.038&7.258 \\
lowThrust\_5&16262&16262&12&12.198&70.124&12&12.198&70.124 \\
hangGlider\_5&16011&16011&8&9.696&112.427&8&9.696&112.427 \\
hangGlider\_4&15561&15561&8&9.609&110.835&8&9.609&110.835 \\
OPF\_3754&15435&15435&9&10.254&5.531&9&10.254&5.531 \\
c-46&14913&14913&7&8.744&42.022&7&8.744&42.022 \\
case9&14453&14453&7&10.238&105.257&7&10.238&105.257 \\
lowThrust\_4&13562&13562&12&11.867&64.031&12&11.867&64.031 \\
lpi\_gosh&13356&3662&9&7.474&5.231&9&27.260&5.231 \\
c-45&13206&13206&5&13.210&85.104&5&13.210&85.104 \\
ca-HepPh&11670&10514&5&20.181&47.173&6&22.400&47.173 \\
coupled&11341&11317&5&8.685&30.083&5&8.704&30.083 \\
c-43&11125&11125&5&11.117&72.602&5&11.117&72.602 \\
psse0&11028&26694&8&9.286&6.075&4&3.836&6.075 \\
psse2&11028&28632&10&10.452&6.713&4&4.026&6.713 \\
c-42&10471&10471&6&10.532&41.339&6&10.532&41.339 \\
nsir&10055&4450&2&15.409&25.894&3&34.817&25.894 \\
c-39&9271&9271&4&14.757&41.233&4&14.757&41.233 \\
wiki-Vote&2355&3728&34&43.018&40.735&8&27.175&40.735 \\
cari&1200&400&1&127.333&178.662&382&382.000&178.662 \\
\end{longtable}
\end{small}

